Frivolous Units: Wider Networks Are Not Really That Wide

A remarkable characteristic of overparameterized deep neural networks (DNNs) is that their accuracy does not degrade when the network's width is increased. Recent evidence suggests that developing compressible representations is key for adjusting the complexity of large networks to the learning task at hand. However, these compressible representations are poorly understood. A promising strand of research inspired from biology is understanding representations at the unit level as it offers a more granular and intuitive interpretation of the neural mechanisms. In order to better understand what facilitates increases in width without decreases in accuracy, we ask: Are there mechanisms at the unit level by which networks control their effective complexity as their width is increased? If so, how do these depend on the architecture, dataset, and training parameters? We identify two distinct types of "frivolous" units that proliferate when the network's width is increased: prunable units which can be dropped out of the network without significant change to the output and redundant units whose activities can be expressed as a linear combination of others. These units imply complexity constraints as the function the network represents could be expressed by a network without them. We also identify how the development of these units can be influenced by architecture and a number of training factors. Together, these results help to explain why the accuracy of DNNs does not degrade when width is increased and highlight the importance of frivolous units toward understanding implicit regularization in DNNs.

==> Frivolous-AAAI-source(1)/abstract.tex <==

%A remarkable characteristic of overparameterized deep neural networks is that their accuracy does not degrade when the network's width is increased. Recent evidence suggests that developing compressible representations is key for adjusting the complexity of large networks to the learning task at hand~\cite{arora2018stronger, zhou2018non, suzuki2019compression}. At the unit level, however, these representations are poorly understood. A better understanding of what compressible features form amongst units will enable a more granular interpretation of the representations in overparameterized networks. Are there mechanisms at the unit level by which networks control their effective complexity? If so, how do these depend on the architecture, dataset, and training parameters?

%We identify two distinct types of ``frivolous'' units that proliferate when the network's width is increased: prunable units which can be dropped out of the network without significant change to the output and redundant units whose activities can be expressed as a linear combination of others. These units imply complexity constraints as the function the network represents could be expressed by a network without them. These results help to explain non-overfitting by showing that overparameterized networks consistently implicitly regularize via the formation of these frivolous units.

% A remarkable characteristic of overparameterized deep neural networks is that their accuracy does not degrade when the network's width is increased. Recent evidence suggests that developing compressible representations is key for adjusting the complexity of large networks to the learning task at hand~\cite{arora2018stronger, zhou2018non, suzuki2019compression}. However, the mechanisms underlying how information representations in network units give rise to generalization remain unclear. A better understanding of what compressible features form at the level of individual units will enable a more granular interpretation of the representations in overparameterized networks and the design of better models. Are there mechanisms reflected at the unit level by which networks control their effective complexity? If so, how do such mechanisms depend on the architecture, dataset, and training parameters? We identify two distinct types of ``frivolous'' units that proliferate when the network's width is increased: \emph{prunable} units which can be dropped out of the network without significant change to the output, and \emph{redundant} units whose activities can be expressed as a linear combination of others. The observation that the network representation could be expressed without ``frivolous'' (prunable and redundant) units. These results help to explain how networks generalize by showing that overparameterized networks consistently auto-regularize via the formation of these frivolous units. 




%Title: Frivolous Units Help to Explain Why the Accuracy of DNNs does not Degrade when the Network's Width is Increased 

%Frivolous units help to explain implicit regularization in deep networks.

%Frivolous units help to explain how overparameterized/wide deep networks constrain their complexity.

% [Boring but possible] Frivolous units emerge in overparameterized deep networks.

%Be Frivolous: Increasing the Network's Width without Degrading the Accuracy

%Be Frivolous: How to increase a network's width without decreasing accuracy

% Frivolous Units: Wider Networks are not really \emph{that} Wide
%(confusable with general compresion work)

% Frivolous units: When Increasing the Network's Width is not Really an Increase
%(not strictly true)

% Frivolous units: complexity increases lag behind width increases in deep networks

A remarkable characteristic of overparameterized deep neural networks (DNNs) is that their accuracy does not degrade when the network width is increased. Recent evidence suggests that developing compressible representations allows the complexity of large networks to be adjusted for the learning task at hand. However, these representations are poorly understood. A promising strand of research inspired from biology involves studying representations at the unit level as it offers a more granular interpretation of the neural mechanisms. In order to better understand what facilitates increases in width without decreases in accuracy, we ask: Are there mechanisms at the unit level by which networks control their effective complexity? If so, how do these depend on the architecture, dataset, and hyperparameters? 

We identify two distinct types of ``frivolous'' units that proliferate when the network's width increases: prunable units which can be dropped out of the network without significant change to the output and redundant units whose activities can be expressed as a linear combination of others. These units imply complexity constraints as the function the network computes could be expressed without them. We also identify how the development of these units can be influenced by architecture and a number of training factors. Together, these results help to explain why the accuracy of DNNs does not degrade when width is increased and highlight the importance of frivolous units toward understanding implicit regularization in DNNs.

% We also identify a number of training factors by which networks can be made to develop more prunable or more redundant units. 



% We also identify several ways in which networks can be trained in order to control what types of frivolous units they develop.
%and investigate how these units affect interpretability in deep networks. 

%remains an open question how  compressibility at the unit level alone is insufficient to predict the generalization abilities of the DNN, it . This highlights that the implicit regularizer of DNNs drives the emergence of  also demonstrate that  .


%by showing that overparameterized networks consistently implicitly regularize via the formation of these frivolous units.


% A remarkable characteristic of overparameterized deep neural networks is that their accuracy does not degrade when the network's width is increased. Recent evidence suggests that developing compressible representations is key for adjusting the complexity of large networks to the learning task at hand~\cite{arora2018stronger, zhou2018non, suzuki2019compression}. The mechanisms underlying how information representation in network units give rise to generalization remain unclear. A better understanding of what compressible features form at the level of individual units will enable a more granular interpretation of the representations in overparameterized networks and the design of better networks. Are there mechanisms reflected at the unit level by which networks control their effective complexity? If so, how do such mechanisms depend on the architecture, dataset, and training parameters? We identify two distinct types of ``frivolous'' units that proliferate when the network's width is increased: \emph{prunable} units which can be dropped out of the network without significant change to the output, and \emph{redundant} units whose activities can be expressed as a linear combination of others. The observation that the network representation could be expressed without ``frivolous'' (prunable and redundant) units suggests specific mechanisms by which compressibility and generalization can be induced. These results help to explain how networks generalize by showing that overparameterized networks consistently auto-regularize via the formation of these frivolous units. 

% Answering these questions will enable a more granular and simple interpretation of the representations in overparameterized networks. 


%In a series of experiments, we show that DNNs consistently increase the number of prunable and redundant units at a rate which outpaces that of other units when width is increased for a comprehensive set of hyperparameters. 


%Deep neural networks (DNNs) perform well on a variety of tasks despite the fact that most networks used in practice are vastly overparameterized and even capable of perfectly fitting randomly labeled data. Recent evidence suggests that developing compressible representations is key for adjusting the complexity of overparameterized networks to the learning task at hand \cite{arora2018stronger, zhou2018non}. In this paper, we provide new empirical evidence which supports this hypothesis by identifying two types of frivolous units that emerge when the network's width is increased: prunable units which can be dropped out of the network without significant change to the output and redundant units whose activities can be expressed as a linear combination of other units. The emergence of these units implies capacity constraints as the function the network represents could be expressed by a smaller network without these units. In a series of experiments with AlexNet, ResNet, and Inception networks in the CIFAR-10 and ImageNet datasets, and also using shallow networks with synthetic data, we show that DNNs consistently increase the number of prunable and redundant units at a rate greater that of other units when width is increased for a comprehensive set of hyperparameters. These results suggest that the mechanisms by which networks in the deep learning regime adjust their complexity operate at the unit level.


==> Frivolous-AAAI-source(1)/broader_impact.tex <==
% In order to provide a balanced perspective, authors are required to include a statement of the potential broader impact of their work, including its ethical aspects and future societal consequences. Authors should take care to discuss both positive and negative outcomes.

% This work provides insights about one of the fundamental properties of deep networks: their ability to generalize to unseen data. Although this is a form of basic research, many practical applications of deep networks require the ability to robustly generalize to novel data without overfitting. This work may contribute to consequential progress in three areas:
% (1) Designing more robust networks: understanding the mechanisms of prunability and redundancy can lead to the design of networks that more reliably implicitly regularize and generalize to reduce risks of system failure. This is widely desirable for improving performance in systems.
% (2) Interpretability: knowledge of frivolous units is helpful for interpreting networks at the unit level. Thus, these results contribute to an improved ability toward the assurance and verification of learning systems. We expect this to be primarily beneficial--especially for systems deployed in safety-critical settings. 
% (3) Compression: we suggest directions for future work in advancing compression techniques which could improve space and time efficiency in deep learning models. This is of particular interest to mobile and web development and could make these systems significantly more accessible. 

% Importantly, the primary factor for how basic research like this will impact society overall is whether the systems which result from it are used responsibly. We join with others in the research community calling for the safe and judicious use of AI in ways that benefit all of humanity. 

This work may contribute to consequential progress in three areas:
(1) \textit{Designing robust networks:} understanding how prunability and redundancy emerge allows for more control over what types of representations they develop. This may lead to insights on improving network design and training.
(2) \textit{Interpretability:} knowledge of frivolous units is helpful for interpreting networks at the unit level which can be valuable for developing a more basic understanding and for verifying properties of learning systems regarding performance or robustness. We expect this to be primarily beneficial, especially for systems in safety-critical settings. 
(3) \textit{Compression:} our findings suggest directions for work in advancing compression techniques which could improve space and time efficiency in deep learning models. This is of particular interest to mobile and web development and could make these systems significantly more accessible. However, this may come with concerns involving the reliability of these systems or their proliferation outpacing effective oversight.

We join with others in the research community calling for the safe and judicious use of AI in ways that benefit all of humanity. 


==> Frivolous-AAAI-source(1)/discussion.tex <==

We have analyzed the emergence of prunable and redundant units in relation to the fact that the generalization ability of DNNs does not tend to decrease as network width increases. Our results show that the number of prunable and/or redundant units increases at a rate which outpaces that of the network overall which suggests that complexity-constraining features in deep networks emerge largely at the unit level. Thus, we offer the following hypothesis: consider a narrow deep network $\mathcal{N}$ and a wide one $\mathcal{W}$, both with the same architecture, trained on the same data with the same regularization and initialization schemata, and each with a tuned set of hyperparameters. Alongside $\mathcal{W}$ generalizing as well or better than $\mathcal{N}$, $\mathcal{W}$ will develop an increased proportion of prunable and/or redundant units relative to $\mathcal{N}$ due to implicit regularization. We hope that future work extending or challenging this hypothesis will lead to a richer understanding of the emergent properties of DNNs.

Despite much recent progress, to our knowledge, this is the first work to date that has quantitatively studied prunability and redundancy together in context of implicit regularization. These methods which target multiple compressible features could be used to improve upon compression based bounds~\cite{arora2018stronger} including for approaches such as that of \cite{zhou2018non} which only considers prunability but not redundancy. We also reveal specific architectures, initializations, and training methods that can be used to control what types of compressible features networks develop. Nonetheless, the fact that both of these types of units consistently proliferate highlights a need for hybrid compression methods which target both.

%The framework used here can also be useful for understanding questions about robustness and redundancy in neuroscience. Given that brains are often surprisingly capable of recovering from damage and neuronal death, it is understood that they are both highly prunable and have built-in redundancies \cite{strehler1980randomness, glassman1987hypothesis}. In fact, Glassman \cite{glassman1987hypothesis} estimates that at least half of the neurons in the human brain fit under our definition of frivolous. Several works have aimed to understand these phenomena in brains using artificial networks as models \cite{schuster2008robust, aerts2016brain, hammelman2016artificial}, but to our knowledge, none have aimed to disentangle prunable from redundant neurons in biological brains. This may be a valuable framework for continued research involving the neuroscience of memory.


%The framework used here can also be useful for understanding questions about robustness and redundancy in neuroscience. This is because the neural activity of DNNs for object recognition has been shown to resemble the neural activity in the brain in areas responsible for this task~\cite{yamins2016using}, and also because brains are often surprisingly capable of recovering from damage and neuronal death, given that neurons are both highly prunable and have built-in redundancies~\cite{strehler1980randomness, glassman1987hypothesis}. In fact, Glassman \cite{glassman1987hypothesis} estimates that at least half of the neurons in the human brain fit under our definition of frivolous. Thus, the hypothesis presented in this paper could be helpful to understand how biological neural networks autoregulate despite being highly overparameterized as artificial DNNs.


The framework used here can also be useful for understanding questions about complexity, robustness, and redundancy in neuroscience. Given that brains are often surprisingly capable of recovering from damage and neuronal death, it is understood that they are overparameterized networks which are both highly prunable and have built-in redundancies \cite{strehler1980randomness}. In fact, \citet{glassman1987hypothesis} estimates that at least half of the neurons in the human brain fit under our definition of frivolous. The neural activity of DNNs for object recognition has been shown to resemble neural activity in parts of the brain~\cite{yamins2016using}, and several works have aimed to understand redundancy and robustness in brains using artificial networks as models~\cite{schuster2008robust, aerts2016brain, hammelman2016artificial}. Thus, the framework presented in this paper could be helpful to understand prunability and redundancy in brains and how biological networks implicitly regularize.


%have been show to Several works have aimed to understand these phenomena in brains using artificial networks as models \cite{schuster2008robust, aerts2016brain, hammelman2016artificial}, but to our knowledge, none have aimed to disentangle prunable from redundant neurons in biological brains. This may be a valuable framework for continued research involving the neuroscience of memory.


While we find that frivolous units are necessary to understand implicit regularization, we do not find that they are sufficient. Although non-frivolous units increase with width at a smaller rate, they increase nonetheless. Future work should investigate the causal factors behind the formation of frivolous units and expand on understanding simplicity in network representations using insights from 
% additional types of compressible motifs derived from other techniques such as 
network distillation \citep{hinton2015distilling}, subnetwork analysis, or 
kernel-inspired analysis~\cite{jacot2018neural}.
% Gaussian processes
Nonetheless, frivolous units play a key role in how networks constrain their effective complexity and offer a milestone toward understanding them at the unit level.


==> Frivolous-AAAI-source(1)/hypothesis.tex <==

Here, we introduce unit-level mechanisms that facilitate increases in network width without decreases in accuracy. We demonstrate that these lead to a function computed by the wider network that can be well-approximated by a thinner one and hence help to explain how performance does not degrade with width. Let $\mathcal{N}$ and $\mathcal{W}$ denote respectively a narrow and a wide DNN with the same architecture which represent mappings from datapoints to labels denoted as $f_\mathcal{N}$ and $f_\mathcal{W}$. Thus, to explain how $\mathcal{W}$ does not utilize its full capacity, we show that $f_\mathcal{W}$ can be expressed with a thinner network,~\ie $f_\mathcal{W} \approx f_\mathcal{N}$ with respect to a data distribution.

To investigate what representations $\mathcal{W}$ develops to facilitate that $f_\mathcal{W} \approx f_\mathcal{N}$, we introduce prunable units which can be removed from a network by excision and redundant units which can be removed by factorizing their layers. Furthermore, we show that these units are distinct and can emerge independently of one another. Similar motifs have been targeted by previous compression works which focus on finding smaller networks that have similar accuracy to an uncompressed one. In contrast, we focus on showing that smaller networks exist which compute similar \emph{functions} as a larger network,~\ie $f_\mathcal{W} \approx f_\mathcal{N}$ across a data distribution. This is more stringent than evaluating accuracy, as preserving accuracy is necessary for showing $f_\mathcal{W} \approx f_\mathcal{N}$ but not sufficient. 
% In the following, we introduce the two types of frivolous units: prunable and redundant.


%\subsection{Frivolous Units} 

\noindent \textbf{\emph{Prunable Units.} }
%Sparsity amongst unit activations in a network is common in biological models and is promoted by linear-threshold activation functions \citep{glorot2011deep, xu2015empirical}. 
Several algorithms based on pruning have been used to compress networks to a fraction of the original size while maintaining test accuracy \cite{han2015deep, han2015learning, hu2016network, luo2017thinet}. The fact that DNNs are robust to the removal of certain units suggests that they compute functions that have a lower complexity than their architectures are capable of.

%A similar criterion was used in the compression algorithm developed by \cite{hu2016network} for identifying individually prunable units. 

Suppose that a narrow network, $\mathcal{N}$, is identical to a wide one, $\mathcal{W}$, but with a set of units removed and that $f_\mathcal{W} \approx f_\mathcal{N}$ across a data distribution. If so, then we refer to the removed units as \emph{prunable}. Note that, due to interactive effects from multiple units, joint and individual prunability are distinct. A variety of phenomena could result in prunability ranging from simple explanations such as units being sparsely activated or their outgoing weights being small, to more complex ones such as subsequent layers discarding their activity.

To evaluate how well removing a set of units preserves network function, we analyze the proportion of examples in a testing set whose labels do not change when units are ablated. Finding the largest set of units that can be removed from a network in a way that results in a given proportion of unchanged labels is NP-hard. Instead of searching for optimal prunable sets, to scalably measure how prunable units are on average, we analyze the proportion of unchanged labels when random ablations are applied to various numbers of units (see Section~\ref{subsec:measures} for details). Fig.~\ref{fig:concept_examples}a-b shows these results. As more units are removed, more output labels change for all networks, however, they exhibit different trends. Fig.~\ref{fig:concept_examples}a shows a case in which the labels output by wider networks are more resistant to random ablations than thinner networks. This indicates that in this case, much of the wider networks' excess capacity goes toward prunable units. Contrastingly, Fig.~\ref{fig:concept_examples}b shows a case in which there is significantly less increase in robustness in a set of networks that only differ from those in Fig.~\ref{fig:concept_examples}a by how they were initialized. However, both types of networks maintain their performance when width is increased as shown in Fig.~\ref{fig:testaccuracy}, suggesting that the networks in Fig.~\ref{fig:concept_examples}b may be developing different capacity constraints. This motivates the search for a second mechanism by which complexity constraints can be understood at the unit level. 

\input{tex_figures/table_networks.tex}


\noindent \textbf{\emph{Redundant Units.}} In contrast to compression algorithms based on pruning are ones which focus on low-rank factorization. These methods in practice have successfully compressed networks to a fraction of their original size while maintaining testing accuracy~\cite{sainath2013low, denton2014exploiting, srinivas2015data}. Most previous works using these methods compress units by representing them in weight space, but units can similarly be represented in activation space across a dataset. 
%Layers in a network can be compressed accordingly so that they only contain a set of basis units whose outgoing weights have been refactored to capture the behavior of other \emph{redundant} units whose activations were approximately linearly dependent on the basis. We provide algorithmic details in the Appendix. Redundant units help to regulate the complexity of the network because removing them via refactorization maintains that $f_\mathcal{W} \approx f_\mathcal{N}$ across the dataset.
We denote as \emph{non-redundant} the largest set of units whose activations are linearly independent (though in experiments we relax this via PCA). The number of non-redundant units is equal to the rank of a matrix that represents the activations of the units across a dataset. The remaining \emph{redundant} units help to regulate the complexity of the network because a thinner network can be constructed without them such that $f_\mathcal{W} \approx f_\mathcal{N}$ across the dataset. In the Appendix, we provide algorithmic details for removing the redundant units and refactoring the outgoing weights of the non-redundant ones.

As with prunability, networks sometimes develop very different levels of redundancy at different widths. Fig.~\ref{fig:concept_examples}c-d depicts the distributions of absolute-valued unit-to-unit correlation coefficients for the final convolutional layers in two classes of networks which only differ in how they were initialized. Fig.~\ref{fig:concept_examples}c shows a case in which the level of unit-to-unit correlation increases only slightly as network width is increased. However, Fig.~\ref{fig:concept_examples}d shows a case in which much more correlation develops with wider networks. Correspondingly, these networks develop more redundant units (see Section~\ref{subsec:measures} for further details). This implies that here, excess capacity is largely utilized to form these redundant units.

%In the Appendix, we give algorithmic details for removing the redundant units and refactoring the outgoing weights of the non-redundant ones.

% \textbf{Redundant Units.} In contrast to compression algorithms based on pruning are ones which focus on low-rank factorization. These methods in practice have successfully compressed networks to a fraction of their original size while maintaining testing accuracy~\cite{sainath2013low, denton2014exploiting, srinivas2015data}. Most previous works using these methods compress units by representing them in weight space, but units can similarly be represented in activation space across a dataset. Layers in a network can be compressed accordingly so that they only contain a set of basis units whose outgoing weights have been refactored to capture the behavior of other \emph{redundant} units whose activations were linearly dependent on the basis. We provide algorithmic details in the Appendix. Redundant units help to regulate the complexity of the network because removing them via refactorization maintains that $f_\mathcal{W} \approx f_\mathcal{N}$ across the dataset.

%Units in a layer can be compressed accordingly so that they only contain a set of basis units whose outgoing weights have been refactored to capture the behavior of other \emph{redundant} units whose activations were linearly dependent on the basis. We provide algorithmic details in the Appendix. Redundant units help to regulate the complexity of the network because removing them via refactorization maintains that $f_\mathcal{W} \approx f_\mathcal{N}$ across the dataset.

%   Also, the expected number of redundant units in randomly initialized networks will be proportional the the network size for large datasets
% \iffalse
% Analogously to prunable units, 
% %$f_\mathcal{W} \approx f_\mathcal{N}$ does not necessarily imply that redundant units {must} exist in $\mathcal{W}$, and 
% the expected number of redundant units in randomly-connected networks will be proportional to the network width (see Appendix). However, trained networks sometimes develop strikingly different levels of redundancy at different width factors. To show this intuitively, 
% \fi

\subsection{Relating Prunable and Redundant Units} \label{subsec_relating}


As reflected in Fig.~\ref{fig:concept_examples}, we clarify here that prunability and redundancy are distinct and prove by construction that they can emerge either together or independently. %We also show that a wide network can compute the same function as a thin one without either type of unit, but we reserve this for the Appendix. 
Recall that $\mathcal{N}$ and $\mathcal{W}$ denote respectively a narrow and a wide DNN with the same architecture and that each represents a mapping from datapoints to labels denoted by $f_\mathcal{N}$ and $f_\mathcal{W}$. Let $\rvu$ refer to the activity of the layer before the output layer in $\mathcal{N}$ and $\boldsymbol\theta$ the incoming weights for the output layer of $\mathcal{N}$. Thus, the output of $\mathcal{N}$ is equal to $\boldsymbol\theta^T\rvu$. Examples can be constructed of a wide network $\mathcal{W}$, twice the size of $\mathcal{N}$, such that $ f_\mathcal{N}=f_\mathcal{W}$ (not only approximately, but exactly) yet each $\mathcal{W}$ has different levels of prunability and redundancy. Note that there are other possible cases aside from the prototypes presented here.

\noindent \textbf{\emph{More of Both Prunable and Redundant Units.}} We can build a $\mathcal{W}$ to be more prunable and redundant by first duplicating the final layer of $\mathcal{N}$ such that the layer before the output has activity $[\rvu, \rvu]$ and setting the output weights equal to $[{\boldsymbol\theta},\boldsymbol{0}]$. Because $[{\boldsymbol\theta},\boldsymbol{0}]^T[\rvu, \rvu]=\boldsymbol\theta^T\rvu$, the outputs will be identical to $\mathcal{N}$. All other layers of $\mathcal{W}$ can then be constructed analogously in the order of deeper to shallower layers. In this case, both prunable and redundant units would be greater in quantity in $\mathcal{W}$ because half of the units in the network are redundant with the other half and can be pruned due to having $\mathbf{0}$-valued outgoing weights. 
%Another example would be constructing $\mathcal{W}$ with the units in $\mathcal{N}$ and with units whose activity is always $0$ because such unresponsive units are prunable and have no activity. 

\noindent \textbf{\emph{Only More Prunable Units.}} A $\mathcal{W}$ that is more prunable but not more redundant can be constructed by first making the units before the output layer in $\mathcal{W}$ equal to $[\rvu, \rvv]$, where $\rvv$ gives units with activities orthogonal to $\rvu$ and each other across the data distribution. Thus, the units are not redundant. To make $f_\mathcal{W}$ equivalent to $f_\mathcal{N}$, the outgoing weights of this layer can be set equal to $[\boldsymbol\theta,\boldsymbol{0}]$, and as in the previous case, the units that are multiplied by $0$ (half of the layer) are prunable. Then constructing other layers analogously from deeper to shallower layers results in a $\mathcal{W}$ that is only more prunable.

\noindent \textbf{\emph{Only More Redundant Units.}} We can duplicate the final layer of $\mathcal{N}$ so that $\mathcal{W}$'s final layer has activations equal to $[\rvu, \rvu]$, making half of the units redundant. Then we can obtain a network that computes the same function as $\mathcal{N}$ via ``weight balancing'' with weights leading into the output layer of $\frac{1}{2}[\boldsymbol\theta + b, \boldsymbol\theta - b]$, where $b$ is a large constant. Although $\frac{1}{2}[\boldsymbol\theta + b,\boldsymbol\theta - b]^T[\rvu, \rvu] = \boldsymbol\theta^T\rvu$, when a unit is pruned, the layer's output changes by an offset of $\frac{1}{2}(b - \theta_k)u_k$, where $u_k$ is the removed unit activation, making it not prunable when $b$ is sufficiently large. Then $\mathcal{W}$ can be completed to be only more redundant by performing the same procedure on on the rest of the network from deeper to shallower layers.

\noindent \textbf{\emph{Upshot.}} Finally, it is helpful to note that $f_\mathcal{W} \approx f_\mathcal{N}$ does not necessarily imply that frivolous units {must} exist in $\mathcal{W}$ because capacity constraints need not emerge at the unit level, and circuits of different complexity can still compute similar functions. We provide clarifying examples in the Appendix. Also in the Appendix, we show that for randomly initialized networks, prunability and redundancy will, in expectation, be proportional to the network width. However, it remains unclear precisely how they emerge in trained networks. As we will show in the following sections, the growth of frivolous units tends to outpace the growth of a network as a whole. 
% Thus, it is unclear if this will also be the case for trained networks, even though for some network such as randomly connected networks,  prunability and redundancy is expected to increase as the width increases (see Appendix). 

==> Frivolous-AAAI-source(1)/introduction.tex <==

%Deep neural networks (DNNs) have achieved state-of-the-art performance in a variety of applications, but this success contrasts with how they are often only interpreted at the level of a black box. A major challenge has been understanding what types of internal representations allow them to learn rather than memorize patterns in data. Though networks are commonly trained with large amounts of data, they are typically ``overparameterized,'' often containing a number of free parameters several orders of magnitude greater than the number of training examples. One striking feature of overparameterized DNNs is that wider networks with more units in each layer tend to generalize as well or better than thinner ones when trained without explicit regularization on the same data, despite having a greater potential for overfitting~\cite{neyshabur2017exploring, neyshabur2018role, Novak2018, poggio2017theory}. This phenomenon by which networks adjust their complexity to avoid overfitting is known as \emph{implicit regularization} and is demonstrated in Fig.~\ref{fig:testaccuracy}. We plot the testing accuracy of common network architectures trained in ImageNet and CIFAR-10 while varying each network's width (see section~\ref{sec_methods} for details). We vary the number of units in fully connected layers and filters in convolutional layers by a size factor. For each architecture, the test errors of wider, more overparameterized, networks do not degrade relative to thinner ones.

A striking feature of deep neural networks (DNNs) is that wider networks with more units in each layer tend to generalize as well or better than thinner ones, even when trained without explicit regularization. In practice, these networks are typically overparameterized,~\ie the number of free parameters is often several orders of magnitude greater than the number of training examples, yet wide versions avoid overfitting relative to thinner ones~\cite{neyshabur2017exploring, neyshabur2018role, Novak2018, poggio2017theory}. This phenomenon is demonstrated in Fig.~\ref{fig:testaccuracy}, in which we plot the testing accuracy of common overparameterized architectures while varying each network's width (see section~\ref{sec_methods} for details). We vary the number of units in fully connected layers and filters in convolutional layers by a size factor. The test errors of wider, more overparameterized networks do not degrade relative to thinner ones, despite a greater potential for overfitting.


\input{tex_figures/accuracy_test.tex}


\citet{frankle2018lottery} find that in certain DNNs, the crucial computations are performed by weight-sparse subnetworks with initializations primed for the learning task,~\ie such subnetworks have won the ``initialization lottery.'' They suggest that wide networks may perform as well as or better than thin ones because they ``buy more lottery tickets'' and more reliably contain these fortuitously initialized subnetworks. However, regarding subnetworks that are not part of a winning ticket, it remains unclear why they do not have a harmful effect on test performance. Some clues may come from recent works involving compression-based performance bounds~\cite{arora2018stronger, zhou2018non, suzuki2019compression}, suggesting a link between compressibility and non-overfitting. This leads to our central question: what neural mechanisms facilitate increases in network width without decreases in accuracy?



%While overparameterized DNNs demonstrably adapt their effective complexity to the given learning task, what mechanisms develop to facilitate this remains an open question. Several signs point to unit-level compressibilities. One example is the success of dropout \cite{srivastava2014dropout}. Other clues come from biological brains which are highly resilient to the death of individual neurons. This is indicative of built-in redundancies and robustness to the loss of individual units, suggesting that many neurons are not necessary for short term performance \cite{strehler1980randomness}. In fact, Glassman \cite{glassman1987hypothesis} estimates that at least half of the neurons in the human brain are not needed! In line with these neuron-focused approaches, a promising strand of research has aimed to understand network representations at the individual unit level~\cite{zeiler2014visualizing, zhou2018revisiting}. Units have been referred to as the ``building blocks of interpretability'' \cite{olah2018building}, as analyzing them allows for simple interpretations of DNNs. For example, individual units act as feature detectors which typically respond to textures or simple patterns at lower layers and more semantically meaningful concepts at higher ones. An open question which remains, however, is how unit-level representations and compressibilities evolve as network width increases. Thus, bridging the gap between unit-level mechanisms and how overparameterized DNNs generalize will allow for an elementary understanding of how they implicitly regularize.


A promising strand of research inspired from neuroscience has aimed to understand network representations at the individual unit level~\cite{zeiler2014visualizing, zhou2018revisiting}. Units have been referred to as the ``building blocks of interpretability''~\cite{olah2018building}, as analyzing them allows for simple interpretations of DNNs. In this paper, we investigate the ways in which unit-level properties evolve as network width increases. Several signs point to compressible units. One example is the success of dropout~\cite{srivastava2014dropout}. Other clues come from biological brains which develop redundancies and are remarkably robust to neuronal death, suggesting that many neurons are not necessary for short-term performance~\cite{strehler1980randomness, glassman1987hypothesis}.
%In fact, Glassman \cite{} estimates that at least half of the neurons in the human brain are not needed.


Here, we identify two types of \emph{frivolous} units which emerge in greater proportions when the network's width is increased: \emph{prunable units} which can be dropped out of the network without significant change to the output, and \emph{redundant units} whose activities can be expressed as a linear combination of others in the same layer. These units are complexity constraints because the function the network represents could be expressed by a thinner network without them. We show that the rate at which these frivolous units appear consistently outpaces the growth of the network as a whole. This suggests that they play a major role in how DNNs constrain their complexity as width is increased. Furthermore, these results add to our understanding of the effects of \emph{implicit regularization} by showing that frivolous units help a network adapt to the complexity of the task at hand.

% add to the growing body of literature that investigates the \emph{implicit regularization} mechanisms in DNNs by showing that frivolous units help to adjust the width of the network to the task at hand.


%Related to this question, it has been shown by Arora~\etal~\cite{arora2018stronger}, Zhou~\etal~\cite{zhou2018non} and Suzuki~\etal~\cite{suzuki2019compression} that networks can often be compressed to thinner versions of themselves with little change in performance and that stronger generalization bounds can be proven for these compressed networks, suggesting a link between compressibility and non-overfitting of wider networks.






==> Frivolous-AAAI-source(1)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvW{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Frivolous-AAAI-source(1)/methods.tex <==

\input{tex_figures/results_imagenet.tex}

Table~\ref{tbl:nets} gives training details. Features we tested multiple variants of are marked with a star ($\star$). Further details for all networks are in the Appendix. To see how  prunability and redundancy vary with width, we tested network variants in which the number of weights/filters in each layer/block/module were multiplied by factors of $1/4$, $1/2$, $1$, $2$, and $4$. 
% For each experiment, we kept training conditions constant including the initialization method across width factors. 

\noindent \textbf{\emph{Datasets.}} For larger scale experiments, we used the ImageNet \cite{ILSVRC15} and CIFAR-10 \cite{krizhevsky2009learning} datasets. For small-scale experiments, we used train and test datasets of 1,000 binary-labeled examples generated by $1/4$x-sized randomly-initialized multilayer perceptrons (MLPs) from uncorrelated Gaussian inputs. We verified these labeling MLPs to output each label for between 40\% and 60\% of inputs. We present results for the test sets, but they were nearly identical for the train sets. 

\noindent \textbf{\emph{Networks.}} For ImageNet, we used ResNet18s from \citet{he2016deep} and Inception-v3 networks from \citet{szegedy2016rethinking}. Due to hardware limitations (we used a dgx1 with 8x NVIDIA V100 GPUs 32GB), we could not train any $2$x or $4$x Inception-v3s and instead experimented with versions with a single layer varied from $1/4$x to $4$x (denoted as \emph{Inception-v3-layer} in plots). For experiments with CIFAR-10, we used AlexNet models based on \citet{Zhang2016} and ResNet56s from \citet{he2016deep}. For small-scale experiments, we used simple MLPs with 1 hidden layer of 128 units for the 1x size. For all networks, increasing model size resulted in equal or improved performance as shown in Fig. \ref{fig:testaccuracy}. In the Appendix, we plot the number of trainable parameters for each network.

\subsection{Measuring Prunability and Redundancy} \label{subsec:measures}

We measure frivolous units via ablation and linear analysis of activations which allows us to experiment with hundreds of networks including convolutional nets at the ImageNet scale. 

\noindent \textbf{\emph{Prunability.} }
% Finding whether or not a set of $n$ units can be removed from a network in way that results in a rate of error corruption of no more than $\epsilon$ across a dataset is NP-hard. Instead of searching for optimal prunable sets, to investigate how prunable the units across a network are on average in a computationally tractable way, 
To measure how prunable units are on average, we analyze robustness to random ablation. We first find what proportion of labels for the test set do not change when varying proportions of units are ablated. These are applied to fully connected layers and feature map outputs in convolutional layers such that each spatial location is treated as a different unit. After obtaining ablation curves as shown in Fig.~\ref{fig:concept_examples}, we use linear interpolation to estimate the proportion of units which can be randomly ablated on average with a tolerance for label corruption of $0.2$ (though trends were similar for different tolerance levels which we tested up to $0.5$). This procedure is repeated three times with randomly chosen units and the set that yields the largest number of prunable units is selected. Finally, we divide by the number of units in the 4x model to normalize the results.

\noindent \textbf{\emph{Redundancy.}} To quantify redundancy, we collect each layer's activation matrix across the test set. In contrast with our method for prunability, for convolutional layers, we treat each feature map output as a unit and consider different spatial locations to be examples for the same unit. We do this because (1) outputs of the same feature map are similar in the sense that they can have the same activity by shifting the image and (2) for computational tractability. We use principal component analysis on the activations to calculate the number of units that are redundant with a tolerance of 0.05 for the proportion of unexplained variance (though trends were similar for different tolerance levels which we tested up to 0.15). We divide by the size of that layer in the 4x model to normalize the results and report the average across all layers of a network weighting each equally regardless of size. 


==> Frivolous-AAAI-source(1)/previous.tex <==
% This work lies at the intersection of three areas of research involving DNNs: understanding implicit regularization, interpreting units, and network compression.


% \iffalse
% \subsection{Understanding Generalization}

% DNNs in certain settings have been shown to exhibit a ``double descent'' phenomenon~\cite{mei2019generalization, nakkiran2019deep, d2020double}. As the width of a DNN increases from one unit per layer, the network's testing loss decreases initially, increases as the complexity approaches that of the training set, and then decreases again. In the second descent where DNNs are overparameterized, they consistently maintain or improve performance despite becoming more expressive. Instead of focusing on the broader question of why DNNs generalize, we focus on this subproblem of understanding how performance does not degrade with increases in model complexity.

% Nonetheless, there is a large background literature on generalization. DNNs in practice have been shown to memorize entire datasets with randomized labels~\cite{Zhang2016}, and a number of works have aimed to uncover why, out of the many optima overparameterized networks can reach, they tend toward ones that generalize well~\cite{neyshabur2017exploring, Novak2018, Zhang2017b}. Some of these approaches have been to derive generalization bounds involving weight norms or Rademacher complexity \cite{bartlett2017spectrally, neyshabur2017pac}. It has also been shown that wide DNNs with high-variance initializations are approximate to kernel machines \cite{belkin2018understand, jacot2018neural, liang2018just, chizat2019lazy}, and other generalization bounds have been based on these comparisons \cite{arora2019fine, hu2020simple}. Additional progress has been made by works showing that DNNs fit simple patterns more readily than complex ones during training~\cite{ansuini2019intrinsic, arpit2017closer, gidel2019implicit, derandom}.
% \fi

\noindent{\textbf{\emph{Understanding Implicit Regularization.}}} DNNs exhibit fascinating properties related to generalization including double descent~\cite{mei2019generalization, nakkiran2019deep, d2020double} and the ability memorize entire datasets with random labels while still generalizing well when trained on uncorrupted data~\cite{Zhang2016}. A number of works have aimed to uncover causal mechanisms that explain why, out of the many optima DNNs can reach, they tend toward simple and geometrically smooth solutions that generalize~\cite{kubo2019implicit, neyshabur2017exploring, neyshabur2018role, Zhang2017b, poggio2017theory, Novak2018}. In particular, some have shown that DNNs fit simple patterns more readily than complex ones~\cite{ansuini2019intrinsic, arpit2017closer, gidel2019implicit, derandom}, that deep ReLU networks tend to exhibit ``surprisingly few'' activation patterns~\cite{hanin2019deep, xiong2020number}, and that the intrinsic dimension of common learning tasks is much lower than the number of network parameters~\cite{li2018measuring}. 

Instead of focusing on the broader question of why DNNs generalize, this work relates to the subproblem of understanding how performance does not degrade with increases in width. This question follows in part from the lottery ticket hypothesis~\cite{frankle2018lottery} as it remains unclear how the capacity of wider networks does not degrade accuracy.
%In addition to works in compression (discussed below), some of these have included norm-based complexity measures \cite{bartlett2017spectrally, liang2019fisher} and how simple activation patterns emerge among their units . 

%Beyond the causal factors of implicit regularization, other works related to this have worked to understand ways in which networks develop ``simple'' representations. In addition to works in compression (discussed below), some of these have included norm-based complexity measures \cite{bartlett2017spectrally, liang2019fisher} and how many distinct activation patterns emerge among their units \cite{hanin2019complexity, hanin2019deep, xiong2020number}. 

\input{tex_figures/concept_examples.tex}


\noindent{\textbf{\emph{Understanding Networks at the Unit Level.}}} A promising framework inspired from neuroscience is understanding representations at the unit level because it leads to elementary and intuitive interpretations of the neural mechanisms. In artificial DNNs, these methods tend to focus on analyzing how units respond to data~\citep{zeiler2014visualizing, montavon2018methods}. Much progress has been made in developing semantic interpretations by optimizing inputs to maximize the activations of units \cite{olah2017feature, olah2018building}, ablational analysis both in recognition networks and GANs~\cite{zhou2018revisiting,bau2018gan}, and interpreting units via a dataset of visual semantic concepts~\cite{bau2017network,mu2020compositional}. 
% Here we hope to gain an intuitive understanding of the neural mechanisms that protect the network from degrading the accuracy when increasing its width.
% One notable experiment related to this work was a case in which dissection was used in \cite{bau2017network} to compare interpretability in AlexNet architectures of different widths.  

%The process of interpreting units is difficult because not all lend themselves to clear semantic interpretations, and there is evidence that DNNs contain many units which are not selective to object categories \cite{morcos2018importance}. Nonetheless,

\noindent{\textbf{\emph{Network Compression.}}} Recent evidence suggests that networks develop compressible representations to adjust their complexity to the learning task at hand~\cite{arora2018stronger, zhou2018non, suzuki2019compression}. Broadly speaking, existing compression algorithms fall into four distinct categories: quantization, knowledge distillation, parameter pruning, and low-rank factorization~\cite{cheng2017survey, choudhary2020comprehensive}. Of these, we focus on pruning and low-rank factorization because they both allow for a simple mapping from an overparameterized network to a compressed one with fewer parameters. Several works have studied compression by pruning low-valued weights and have shown that the number of parameters can often be compressed by an order of magnitude or more this way~\cite{fukuyama2014state, molchanov2017variational, tung2018clip, ma2019resnet}. However, weights are more difficult to interpret than units, and these methods prune weights based on magnitude alone without analyzing how the network behaves across a dataset. Contrastingly, the approaches we discuss in the following section are data-driven and unit-centric. 


%We focus on prunable and redundant units as it facilitates intuitive interpretations that extend our understanding at the unit level is partially inspired from compression algorithms.

==> Frivolous-AAAI-source(1)/results.tex <==

\label{results_section}
\label{sec_results}

\input{tex_figures/supp_randomlabels.tex}

Here, we introduce how prunability and redundancy vary as a function of model width across size factors from 1/4x to 4x. We use a $\log$ scale for both axes in all plots and include maximum and minimum ``gain'' values for the curves in each plot represented as $g_{\min}$ and $g_{\max}$. This gain value gives the average increase in the number of prunable and redundant units as network width is doubled. A gain $g > 2$ indicates that a type of unit more-than-doubles on average when the network width is doubled. Excluding Figs.~\ref{fig:imagenet_results}a,c,d, points are averages across three trials. Error bars giving standard deviations are provided, but do not always appear at the given scale. See the Appendix for further details.


\noindent \textbf{{Prunability and/or redundancy increase at a rate greater than units of the network overall.}} Fig.~\ref{fig:imagenet_results}a-b and Fig.~\ref{fig:results_other}a-d show that both types of units consistently emerge across experiments. For all but two cases (redundancy in Inception-v3s and prunability in ResNet56s trained on random labels), $g_{\min} > 2$ meaning that the growth rate of frivolous units is greater than that of the overall network. This demonstrates implicit regularization at the unit level by showing that in wider networks, the distribution of units tends to prefer frivolous ones more than in thinner networks. We also plot trends for the individual layers of ResNet18s in Fig.~\ref{fig:imagenet_results}c-d and Inception-v3s in the Appendix. While frivolous units consistently emerge in individual layers when their width is increased, they do so to varying extents, and we find no consistent relationship between depth and frivolity. 

The fact that frivolous units tend to more-than-double is mirrored by the fact that their non-frivolous ones tend to less-than-double which is shown in the Appendix. We also find that although non-prunable and non-redundant units increase at a lower rate, they increase nonetheless. It is notable that even if the rate of increase is larger for frivolous units, if a network has a small proportion of them to begin with, it can develop more new non-frivolous units than new frivolous ones as width increases. 
% This demonstrates that although prunability and redundancy account for much of the implicit regularization mechanisms of the network, they don't account for all of them. 
This suggests avenues for future work toward understanding non-prunable and non-redundant units using methods other than analysis of prunable and redundant units separately. A promising possibility is analysis of both jointly. Note that in some networks, particularly Inception-v3s and ResNet18s in Fig.~\ref{fig:imagenet_results}a-b, trends in prunability and redundancy differ significantly which demonstrates that these measurements respond to distinct sets of units. 


\noindent \textbf{{Prunability and redundancy develop in networks trained on random labels.}} To better understand the relationship between frivolous units and generalization, we analyze networks trained to memorize randomly labeled images. Fig.~\ref{fig:results_other}a compares the results with AlexNet and ResNet56 models trained with and without random labels. With random labels, all networks of the 1x size or greater fit the training set with at least 99\% accuracy. Even when fitting noise, these models increase the quantity of frivolous units and even increase the number of redundant ones with $g_{\min} > 2$. This demonstrates that although the emergence of frivolous units with $g > 2$ implies implicit regularization, it does not imply generalization.


\input{tex_figures/lucid_vis_small}


\noindent \textbf{{Trends are similar under explicit regularization.}} To compare the effects of implicit and explicit regularization, we ask how explicit regularizers influence the emergence of frivolous units. In Fig.~\ref{fig:results_other}b, we show that data augmentation, dropout, weight decay, and all three together have only modest effects on the trends in frivolous units. This suggests that implicit regularization may operate at the unit level in significantly different ways than explicit regularization. 


\noindent \textbf{{Initialization influences prunability and redundancy.}} Some recent works have suggested that network initialization has a large influence over generalization behavior \cite{frankle2018lottery, chizat2019lazy, woodworth2019kernel}. To analyze its effects on frivolous units, we test three common methods of weight initialization. Fig.~\ref{fig:results_other}c presents results for AlexNets trained with Glorot \citep{glorot2010understanding}, He \citep{he2015delving}, and Lecun \citep{lecun2012efficient} initializations which each initialize weights using Gaussian distributions with variances depending on the layer widths. %of $2/(|Lyr_{i-1}|+|Lyr_{i}|)$, $2/|Lyr_{i-1}|$, and $1/|Lyr_{i-1}|$ 
%$2/(\textrm{fan\_in}+\textrm{fan\_out})$, $2/\textrm{fan\_in}$, and $1/\textrm{fan\_in}$ 
%respectively. 
In these networks, as the initializations change, there is a tradeoff between the emergence prunable and redundant units. We also display the same curves for uniform-distributed versions of these initializations in the Appendix and find the results to be similar, suggesting that the initialization distribution matters little compared to variance. 


\noindent \textbf{{Datasets influence prunability and redundancy.}} To see if frivolous units result from structure in the input data, we train MLPs on uncorrelated data with labels from randomly initialized teacher networks. Fig.~\ref{fig:results_other}d, shows the results of altering initialization variance in MLPs trained on these datasets with examples of 10 and 10,000 dimensions. Results from the full hyperparameter searches are in the Appendix. Despite uncorrelated training data, prunability and redundancy emerge nonetheless with $g > 2$, though not as large as for other experiments. For the case with high initialization variance and high input dimension, the MLPs have similar $g$ values for prunability to other networks but have a much lower number of prunable units. This indicates an interaction between initialization and dataset in the emergence of prunable units. 

\noindent \textbf{{Results are consistent across optimizers, learning rates, batch sizes, and number of training epochs.}} Results from additional experiments are in the Appendix. %We test training MLPs using stochastic gradient descent (SGD), momentum, and Adam. Trends were consistent across optimizers. Additionally, we also vary learning rate and batch size while keeping them proportional in ResNet18, ResNet56, and AlexNet models trained on ImageNet and CIFAR-10 and find that they reinforce our main findings. We also analyze the presence of prunable and redundant units for different amounts of training time after convergence in ResNet18s and show that they are stable. 

% \noindent \textbf{{Frivolous units may not pose major challenges to developing semantic interpretations of units in wide networks.}} 
\noindent \textbf{{Network width influences interpretability but with no consistent trend across layers.}} Given that prunable units do not seem to represent any features essential for the task at hand and that redundant units may be representable as a combination of multiple feature directions, we ask whether these units degrade interpretability in wide networks. To test this, we use Lucid~\cite{olah2017feature} to generate images optimized to maximize the activation of units in 1/4x and 4x ResNet18s and 1/4x and 1x Inception-v3s. Examples from the first block of ResNet-18s are shown in Fig.~\ref{fig:lucid_vis_small} (see Appendix for more visualizations). As a proxy measure for interpretability, we calculate the \emph{total variation} of these visualizations which measures how different the values of adjacent pixels are. The total variations were analyzed both for the raw visualizations and their Fourier transforms (lower total variation means better interpretability). To compare results between thin and wide networks for each block/module, we use a rank-based permutation test. These tests provide evidence that there are differences between the thin and wide networks across layers, but not that the thin ones are consistently more interpretable. Thorough details including a table of $p$ values and effect sizes are in the Appendix.  


==> Frivolous-AAAI-source(1)/tex_figures/ablation.tex <==
\begin{figure}[t!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{0.1cm}}c}
%	\includegraphics[width=.33\linewidth]{figures/rob_imagenet.pdf} &
  \includegraphics[width=.5\linewidth]{figures/rob_cifar.pdf} &
   \includegraphics[width=.5\linewidth]{figures/rob_cifar_init.pdf} \\
	(a) & (b) \\ 
\end{tabular}
\caption{\textbf{Some  networks  develop  more  resistance  to unit removal as model size increases.}  Each point shows the proportion of labels that did not change when the percentage of units on the x-axis were randomly ablated. Networks were identically trained except for initialization and model size. No explicit regularization was used. (a) Glorot-initialized AlexNets in CIFAR-10. (b) He-initialized AlexNets in CIFAR-10.}
\label{fig:ablation}
\end{figure}


\begin{figure}[t!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{0.1cm}}c}
%	\includegraphics[width=.33\linewidth]{figures/rob_imagenet.pdf} &
      	\includegraphics[width=.5\linewidth]{figures/glorot_violins.pdf} &
	\includegraphics[width=.5\linewidth]{figures/he_violins.pdf} \\
	(a) & (b)  \\ 
\end{tabular}
\caption{\textbf{Some networks develop more highly correlated units as model size increases.} Each violin plot shows the distribution of pairwise correlation coefficients for the final convolutional layer of the network across the testing set. Networks were identically trained except for initialization and model size. No explicit regularization was used. (a) Glorot-initialized AlexNets in CIFAR-10. (b) He-initialized AlexNets in CIFAR-10.}
\label{fig:ablation2}
\end{figure}


==> Frivolous-AAAI-source(1)/tex_figures/accuracy_test.tex <==

\begin{figure*}[t!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
    \includegraphics[width=.33\linewidth]{figs/acc_imagenet_test.pdf}&
    \includegraphics[width=.33\linewidth]{figs/acc_cifar_test.pdf}&
	\includegraphics[width=.33\linewidth]{figs/acc_cifar_initializers_test.pdf}\\
	(a) & (b) & (c) \\
\end{tabular}
\caption{Test accuracy does not degrade with model width in overparameterized deep networks. Top-1 test accuracies across model sizes and datasets. (a) ResNet18s, Inception-v3s, and Inception-v3-layer (with a single layer's width varied) trained in ImageNet. (b) Regularized AlexNets and ResNet56s with and without training on random labels in CIFAR-10. (c) Unregularized Alexnet with Glorot, He, or LeCun initialization, in CIFAR-10.}
\label{fig:testaccuracy}
%\vspace{-0.3cm}
\end{figure*}



==> Frivolous-AAAI-source(1)/tex_figures/accuracy_train.tex <==
\begin{figure*}[h!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
	\includegraphics[width=.33\linewidth]{figures/acc_synth_train.pdf}&
	\includegraphics[width=.33\linewidth]{figures/acc_cifar_initializers_train.pdf} &
	\includegraphics[width=.33\linewidth]{figures/acc_imagenet_train.pdf}\\
	(a) & (b) & (c) \\
\end{tabular}
\caption{\textbf{Train accuracies for our featured networks:} Each point represents a mean top-1 accuracy. Error bars are too small to appear at this scale.}
\label{fig:trainaccuracy}
\end{figure*}

==> Frivolous-AAAI-source(1)/tex_figures/auc.tex <==
\begin{figure*}[h!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
	\includegraphics[width=.33\linewidth]{figures/auc_synthetic_test.pdf}&
	\includegraphics[width=.33\linewidth]{figures/auc_cifar_initializers_test.pdf} &
	\includegraphics[width=.33\linewidth]{figures/auc_imagenet_test.pdf}\\
	(a) & (b) & (c) \\
\end{tabular}
\caption{\textbf{Areas under random ablation curves:} For each non-ImageNet network, we trained three replicates, and each point is an average across layers, samplings, and replicates (if applicable). Most error bars are too small to appear at this scale. We attribute the fact that the smallest MLPs did not have 50\% label change after 100 \% ablation to our use of bias terms in each layer.}
\label{fig:auc}
\end{figure*}

==> Frivolous-AAAI-source(1)/tex_figures/compression.tex <==
\begin{figure*}[h!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
	\includegraphics[width=.33\linewidth]{figures/comp_synthetic_test.pdf}&
	\includegraphics[width=.33\linewidth]{figures/comp_cifar_initializers_test.pdf} &
	\includegraphics[width=.33\linewidth]{figures/comp_imagenet_test.pdf}\\
	(a) & (b) & (c) \\
\end{tabular}
\caption{\textbf{Compressibility:} What proportion of principle components (relative to the number of neurons) are needed to explain 95\% of the variance in the neuronal activation vectors. For each non-ImageNet network, we trained three replicates, and each point is an average across layers, samplings, and replicates (if applicable). Most error bars are too small to appear at this scale.}
\label{fig:compression}
\end{figure*}

==> Frivolous-AAAI-source(1)/tex_figures/concept_examples.tex <==
\begin{figure*}[t!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.05cm}}c@{\hspace{-0.05cm}}c@{\hspace{-0.05cm}}c}
    \includegraphics[width=.25\linewidth]{figs/rob_cifar_new.pdf} &
    \includegraphics[width=.25\linewidth]{figs/rob_cifar_init_new.pdf} & 
    \includegraphics[width=.25\linewidth]{figs/glorot_violins_new.pdf} &
	\includegraphics[width=.25\linewidth]{figs/he_violins_new.pdf} \\
	(a) & (b) & (c) & (d) \\ 
\end{tabular}
\caption{Networks develop units which are prunable and units that are linearly dependent to varying degrees. All networks were identically trained AlexNets except for width and  initialization. No explicit regularization was used. Glorot (low-variance) initialized networks are in purple, and He (high-variance) in blue. (a-b) Prunable units: points show the proportion of labels that did not change when the percentage of units on the x-axis was randomly ablated. (c-d) Redundant units: violin plots with absolute-valued correlation coefficients between unit activations for the final convolutional layer across the testing set.}
\label{fig:concept_examples}
\vspace*{-0.35cm}
\end{figure*}


% \begin{figure}[t!]
% \centering
% \begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{0.1cm}}c}
% %	\includegraphics[width=.33\linewidth]{figures/rob_imagenet.pdf} &
%       	\includegraphics[width=.5\linewidth]{figures/glorot_violins.pdf} &
% 	\includegraphics[width=.5\linewidth]{figures/he_violins.pdf} \\
% 	(a) & (b)  \\ 
% \end{tabular}
% \caption{\textbf{Some networks develop more highly correlated units as model size increases.} Each violin plot shows the distribution of pairwise correlation coefficients for the final convolutional layer of the network across the testing set. Networks were identically trained except for initialization and model size. No explicit regularization was used. (a) Glorot-initialized AlexNets in CIFAR-10. (b) He-initialized AlexNets in CIFAR-10.}
% \label{fig:ablation2}
% \end{figure}


==> Frivolous-AAAI-source(1)/tex_figures/layers.tex <==

\begin{figure*}[]
\centering
\begin{tabular}{c@{\hspace{-0.1cm}}c}
	\includegraphics[width=.3\linewidth]{figs/prune_imagenet_inception_all_layer.pdf} &
	% \includegraphics[width=.33\linewidth]{figures/comp_imagenet_layer_inception_test.pdf} &
	\includegraphics[width=.3\linewidth]{figs/red_imagenet_inception_all_layer.pdf} \\
	(a) & (b)\\
\end{tabular} 
\caption{Inception-v3 prunability and redundancy layerwise (ImageNet): Trends in (a) prunability and (b) redundancy among the final $35 \times 35$ (layer 7), $17 \times 17$ (layer 12), and $8 \times 8$ (layer 13) blocks within Inception-v3 in ImageNet. Gains for the individual layers are similar to the network as a whole.}
\label{fig:layerwise_Inception-v3}
\end{figure*}

\begin{figure*}[]
\centering
\begin{tabular}{c@{\hspace{-0.1cm}}c}
	\includegraphics[width=.3\linewidth]{figs/prune_imagenet_inception_layer.pdf} &
	% \includegraphics[width=.33\linewidth]{figures/comp_imagenet_layer_inception_layer_test.pdf} &
	\includegraphics[width=.3\linewidth]{figs/red_imagenet_inception_layer.pdf} \\
	(a) & (b)\\
\end{tabular}
\caption{Inception-v3 single layer prunability and redundancy layerwise (ImageNet): Trends in (a) prunability, and (b) redundancy among the final $35 \times 35$ (layer 7), $17 \times 17$ (layer 12), and $8 \times 8$ (layer 13) blocks within Inception-v3s in ImageNet as only the final $35 \times 35$ layer is varied in size. Varying the size of a single layer has no effect on the unit prunability and redundancy of other layers.}
\label{fig:layerwise_Inception-v3_layer}
\end{figure*}

==> Frivolous-AAAI-source(1)/tex_figures/lucid_vis.tex <==
\begin{figure*}[]
\centering
\begin{tabular}{cc}
    (a) & \includegraphics[width=.92\linewidth]{figs/resnet18_block1_thin_lucid.png} \\
     & \includegraphics[width=.92\linewidth]{figs/resnet18_block1_thin_lucid_fourier.png} \\
     (b) & \includegraphics[width=.92\linewidth]{figs/resnet18_block1_wide_lucid.png} \\
     & \includegraphics[width=.92\linewidth]{figs/resnet18_block1_wide_lucid_fourier.png}\\
    (c) & \includegraphics[width=.92\linewidth]{figs/resnet18_block4_thin_lucid.png} \\
     & \includegraphics[width=.92\linewidth]{figs/resnet18_block4_thin_lucid_fourier.png} \\
     (d) & \includegraphics[width=.92\linewidth]{figs/resnet18_block4_wide_lucid.png} \\
     & \includegraphics[width=.92\linewidth]{figs/resnet18_block4_wide_lucid_fourier.png}
\end{tabular}
\caption{Visualizations in pixel and Fourier space of 8 units from each of the first block (a,b) and final block (c,d) of the 1/4x (a,c) and 4x (b,d) ResNet18s. The total variations of these images were used for hypothesis testing via a rank-based permutation test..} 
\label{fig:lucid_vis}
\end{figure*}



==> Frivolous-AAAI-source(1)/tex_figures/lucid_vis_small.tex <==
\begin{figure*}[]
\centering
\begin{tabular}{cc}
    (a) & \includegraphics[width=.92\linewidth]{figs/resnet18_block1_thin_lucid.png} \\
     (b) & \includegraphics[width=.92\linewidth]{figs/resnet18_block1_wide_lucid.png} \\
\end{tabular}
\caption{Example visualizations of 8 units from the first block of the 1/4x (a) and 4x (b) ResNet-18s. The total variations of these images and their Fourier transforms were used for hypothesis testing via a rank-based permutation test.} 
\label{fig:lucid_vis_small}
\end{figure*}


==> Frivolous-AAAI-source(1)/tex_figures/lucid_vis_table.tex <==
\begin{table*}[h!]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{2pt} % Default value: 6pt
    
    \begin{tabular}{|l|r|r|r|r|}
    \hline
        \cellcolor{Gray} \textbf{ResNet18} & \cellcolor{Gray} Block 1 & \cellcolor{Gray} Block 2 & \cellcolor{Gray} Block 3 & \cellcolor{Gray} Block 4 \\ \hline
        \cellcolor{Gray} Total Var p (Pixel) & 0.751 & 0.835 & 0.563 & \textbf{0.001} \\ 
        \cellcolor{Gray} Mean Effect (Pixel) & 1.027 & 1.171 & 0.987 & 0.883 \\ \hline
        \cellcolor{Gray} Total Var p (Freq) & 0.361 & 0.750 & 0.25 & \textbf{0.001} \\ 
        \cellcolor{Gray} Mean Effect (Freq) & 0.970 & 1.127 & 0.967 & 0.863 \\ \hline
    \end{tabular}\\
    
    \vspace{0.1cm}
    
    \begin{tabular}{|l|r|r|r|r|r|r|}
    \hline
        \cellcolor{Gray} \textbf{Inception-v3} & \cellcolor{Gray} Conv4 & \cellcolor{Gray} 35x35x256a & \cellcolor{Gray} 35x35x288a & \cellcolor{Gray} 35x35x288b & \cellcolor{Gray} 17x17x768a & \cellcolor{Gray} 17x17x768b\\ \hline
        \cellcolor{Gray} Total Var p (Pixel) & \textbf{0.982} & 0.566 & 0.080 & \textbf{0.018} & \textbf{0.990} & 0.140 \\ 
        \cellcolor{Gray} Mean Effect (Pixel) & 1.237 & 1.016 & 0.820 & 0.856 & 1.275 & 0.883 \\ \hline
        \cellcolor{Gray} Total Var p (Freq) & \textbf{0.989} & 0.263 & \textbf{0.019} & 0.065 & \textbf{0.998} & 0.118 \\
        \cellcolor{Gray} Mean Effect (Freq) & 1.406 & 0.983 & 0.831 & 0.875 & 1.324 & 0.920 \\ \hline
        
        \cellcolor{Gray} & \cellcolor{Gray} 17x17x768c & \cellcolor{Gray} 17x17x768d & \cellcolor{Gray} 17x17x768e & \cellcolor{Gray} 17x17x1280a & \cellcolor{Gray} 8x8x2048a & \cellcolor{Gray} 8x8x2048b \\ \hline
        \cellcolor{Gray} Total Var p (Pixel) & 0.097 & 0.116 & 0.520 & \textbf{0.010} & \textbf{0.005} & \textbf{0.004} \\
        \cellcolor{Gray} Mean Effect (Pixel) & 0.900 & 0.898 & 0.977 & 0.858 & 0.884 & 0.814 \\ \hline
        \cellcolor{Gray} Total Var p (Freq) & 0.194 & 0.096 & 0.714 & 0.443 & 0.288 & 0.138 \\
        \cellcolor{Gray} Mean Effect (Freq) & 0.943 & 0.926 & 1.018 & 0.943 & 0.973 & 0.917 \\ \hline
    \end{tabular}
    \caption{One-sided p values and mean effect sizes testing for low total variation among visualizations of thin versus wide networks. Each p value is from rank-based permutation test on 8 units from each network and 100,000 samples. Results are given both for images in pixel and frequency space. A small p value indicates that the visualizations of units in the thinner network have a lower total variation. All p values below 0.025 or above 0.975 are bolded. Each effect size gives the mean total variation for the thin networks divided by the same for the wide networks. A small mean effect means that the thin network's visualizations had a smaller average total variation.}
    \label{tab:vis_pvalues}
\end{table*}
 


==> Frivolous-AAAI-source(1)/tex_figures/non_imagenet.tex <==
\begin{figure*}[]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
  \includegraphics[width=.26\linewidth]{figs/nonprune_imagenet.pdf} &
  \includegraphics[width=.26\linewidth]{figs/nonred_imagenet.pdf} &
    \includegraphics[width=.26\linewidth]{figs/nonprune_imagenet_resnet_all_layer.pdf} &
    \includegraphics[width=.26\linewidth]{figs/nonred_imagenet_resnet_all_layer.pdf}\\
	(a) & (b) & (c) & (d) \\
\end{tabular}
\caption{Non-frivolous units emerge in ResNet18s and Inception-v3s with smaller gains than frivolous ones. (a) Non-prunability. (b) Non-redundancy. (c) Non-prunability layerwise for ResNet18s. (d) Non-redundancy layerwise for ResNet18s. The gain, $g$, gives the increase when the network size is doubled. Max and min $g$ values are given.}
\label{fig:non_imagenet}
\end{figure*}


==> Frivolous-AAAI-source(1)/tex_figures/non_others.tex <==


\begin{figure*}[]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}

    \includegraphics[width=.26\linewidth,valign=T]{figs/nonprune_cifar_rand.pdf} & 
	\includegraphics[width=.26\linewidth,valign=T]{figs/nonprune_cifar_regularizers.pdf}&
	\includegraphics[width=.26\linewidth,valign=T]{figs/nonprune_cifar_initializers.pdf} &
	\includegraphics[width=.26\linewidth,valign=T]{figs/nonprune_synth_summary.pdf}\\

    \includegraphics[width=.26\linewidth]{figs/nonred_cifar_rand.pdf} & 
	\includegraphics[width=.26\linewidth]{figs/nonred_cifar_regularizers.pdf}&
	\includegraphics[width=.26\linewidth]{figs/nonred_cifar_initializers.pdf} &
	\includegraphics[width=.26\linewidth]{figs/nonred_synth_summary.pdf}\\
	
	(a) & (b)& (c)& (d)\\
	
\end{tabular}
\caption{Non-frivolous units emerge with smaller gains than frivolous ones for different architectures, regularizers, initializers and datasets. (a) AlexNets and ResNet56s trained with and without random labels (CIFAR-10). (b) AlexNets trained with and without regularization (CIFAR-10). (c) AlexNets trained with various initializations (CIFAR-10). (d) MLPs with different input sizes and initializations (synthetic data). Max and min gain factors are given for each plot.}
\label{fig:non_other}
\end{figure*}





==> Frivolous-AAAI-source(1)/tex_figures/non_selectivity.tex <==
\begin{figure}[h!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
	\includegraphics[width=.33\linewidth]{figures/noselec_synthetic_test.pdf}&
	\includegraphics[width=.33\linewidth]{figures/noselec_cifar_initializers_test.pdf} &
	\includegraphics[width=.33\linewidth]{figures/nonselec_imagenet_test.pdf}\\
	(a) & (b) & (c) \\
\end{tabular}
\caption{\textbf{Nonselectivity:} Proportions of neurons with a selectivity factor of less than 0.05 where 0 is perfect promiscuity and 1 is perfect selectivity. For each non-ImageNet network, we trained three replicates, and each point is an average across layers, samplings, and replicates (if applicable). Most error bars are too small to appear at this scale.}
\label{fig:nonselectivity}
\end{figure}

==> Frivolous-AAAI-source(1)/tex_figures/parameters.tex <==
\begin{figure*}[]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
	\includegraphics[width=.33\linewidth]{figs/param_synthetic.pdf}&
	\includegraphics[width=.33\linewidth]{figs/param_cifar.pdf} &
	\includegraphics[width=.33\linewidth]{figs/param_imagenet.pdf}\\
	(a) & (b) & (c) \\
\end{tabular}
\caption{Parameters: (a) Multilayer perceptrons, (b) AlexNets and ResNet56s, (c) ResNet18s, Inception-v3s, and Inception-v3s with a single layer varied. The log number of trainable parameters at each model size.}
\label{fig:params}
\end{figure*}

==> Frivolous-AAAI-source(1)/tex_figures/results_cifar.tex <==
\begin{figure}[t!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
  \includegraphics[width=.26\linewidth]{figures/nonprune_imagenet.pdf} &
  \includegraphics[width=.26\linewidth]{figures/nonred_imagenet.pdf} &
    \includegraphics[width=.26\linewidth]{figures/nonprune_cifar_regularizers.pdf} &
    \includegraphics[width=.26\linewidth]{figures/nonred_cifar_regularizers.pdf}\\
	(a) & (b) & (c) & (d)  \\
\end{tabular}
\caption{\textbf{Initialization influences unit removability and repetition.} Glorot initialization leads to repetition without replication, He initialization leads to repetition without removability, and LeCun initialization leads to intermediate results in AlexNets (CIFAR-10) (a) Areas under ablation curves, (b) the average number of similar units per unit. Each point is an average across layers.}

\label{fig:results_cifar}
\end{figure}


==> Frivolous-AAAI-source(1)/tex_figures/results_imagenet.tex <==
\begin{figure*}[]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
  \includegraphics[width=.26\linewidth]{figs/prune_imagenet.pdf} &
  \includegraphics[width=.26\linewidth]{figs/red_imagenet.pdf} &
    \includegraphics[width=.26\linewidth]{figs/prune_imagenet_resnet_all_layer.pdf} &
    \includegraphics[width=.26\linewidth]{figs/red_imagenet_resnet_all_layer.pdf}\\
	(a) & (b) & (c) & (d) \\
\end{tabular}
\caption{Prunability strongly outpaces the growth of the network as a whole and redundancy increases at rates similar to the network in ResNet18s and Inception-v3s. (a) Prunability. (b) Redundancy. (c) Prunability layerwise for ResNet18s. (d) Redundancy layerwise for ResNet18s. The gain, $g$, represents the increase in prunability or redundancy when the network size is doubled. Max and min $g$ values are given for each plot.}
\label{fig:imagenet_results}
\vspace{-0.3cm}
\end{figure*}


==> Frivolous-AAAI-source(1)/tex_figures/results_synthetic.tex <==
\begin{figure}[h!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
	\includegraphics[width=.33\linewidth]{figures/auc_synthetic_test.pdf} & 
	\includegraphics[width=.33\linewidth]{figures/comp_synthetic_test.pdf} & 
	\includegraphics[width=.33\linewidth]{figures/selec_synth_test.pdf}\\
	(a) & (b) & (c) \\
\end{tabular}
\caption{\textbf{Uncorrelated data MLP robustness and redundancy:} (a) Areas under ablation curves. (b) What proportion of principle components (relative to the number of neurons) are needed to explain 95\% of the variance in the neuronal activation vectors. (c) The average number of similar neurons (neurons with a Pearson $abs(r)$ of at least 0.5) per neuron in each model. Each point is an average across layers, samplings, and 3 model replicates. Each point is an average across layers, samplings, and three model replicates. For (a) and (b), error bars are based on replicates and are mostly too small to appear. For (c), error bars represent the average standard deviation of selectivity \emph{within} samplings.}
\label{fig:results_imagenet}
\end{figure}

==> Frivolous-AAAI-source(1)/tex_figures/selectivity.tex <==
\begin{figure}[h!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
	\includegraphics[width=.33\linewidth]{figures/selec_synth_test.pdf}&
	\includegraphics[width=.33\linewidth]{figures/selec_cifar_initializers_test.pdf} &
	\includegraphics[width=.33\linewidth]{figures/selec_imagenet_test.pdf}\\
	(a) & (b) & (c) \\
\end{tabular}
\caption{\textbf{Selectivity:} The average selectivity factor where 0 is perfect promiscuity and 1 is perfect selectivity. For each non-ImageNet network, we trained three replicates, and each point is an average across layers, samplings, and replicates (if applicable). Error bars represent the average standard deviation of selectivity \emph{within} samplings.}
\label{fig:selectivity}
\end{figure}

==> Frivolous-AAAI-source(1)/tex_figures/similarity.tex <==
\begin{figure*}[h!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
	\includegraphics[width=.33\linewidth]{figures/sim_synth_test.pdf}&
	\includegraphics[width=.33\linewidth]{figures/sim_cifar_initializers_test.pdf} &
	\includegraphics[width=.33\linewidth]{figures/sim_imagenet_test.pdf}\\
	(a) & (b) & (c) \\
\end{tabular}
\caption{\textbf{Similarity:} The average number of similar neurons (neurons with a Pearson $abs(r)$ of at least 0.5) per neuron in each model. For each non-ImageNet network, we trained three replicates, and each point is an average across layers, samplings, and replicates (if applicable). Error bars represent the average standard deviation of similarity \emph{within} samplings.}
\label{fig:similarity}
\end{figure*}

==> Frivolous-AAAI-source(1)/tex_figures/supp_batch_cifar.tex <==
\begin{figure*}[]
\centering
\begin{tabular}{ccc}
	\includegraphics[width=.3\linewidth]{figs/acc_cifar_batch_test.pdf}&
	\includegraphics[width=.3\linewidth]{figs/prune_cifar_batch.pdf}&
	% \includegraphics[width=.3\linewidth]{figures/comp_cifar_batch_test.pdf} & 
	\includegraphics[width=.3\linewidth]{figs/red_cifar_batch.pdf}\\
	(a) & (b) & (c)\\
\end{tabular}
\caption{Trends in accuracy and frivolous units do not depend on learning rate and batch size in networks trained on CIFAR-10. Trends in (a) accuracy, (b) prunability, and (c) redundancy across model sizes for AlexNets and ResNet56s. We vary a constant factor $k$ from $1/4$ to $4$ as a multiplier for the batch sizes and learning rates. 4x AlexNets with $k=4$ were not trained due to hardware restrictions. }
\label{fig:batch_cifar}
\end{figure*}



==> Frivolous-AAAI-source(1)/tex_figures/supp_batch_imagenet.tex <==
\begin{figure*}[h!]
\centering
\begin{tabular}{ccc}
	\includegraphics[width=.3\linewidth]{figs/acc_imagenet_batch_test.pdf}&
	\includegraphics[width=.3\linewidth]{figs/prune_imagenet_batch.pdf}&
	% \includegraphics[width=.4\linewidth]{figures/comp_imagenet_batch_test.pdf}&
	\includegraphics[width=.3\linewidth]{figs/red_imagenet_batch.pdf} \\
	(a) & (b) & (c)\\
\end{tabular}
\caption{Trends in accuracy and frivolous units do not depend on learning rate and batch size factor in ResNet18s trained in ImageNet. Trends in (a) accuracy, (b) prunability, and (c) redundancy across model sizes. We vary a constant factor $k$ from $1/4$ to $4$ as a multiplier for the batch sizes and learning rates. ``Max'' refers to the maximum batch size that could be used for training a model given available hardware (dgx1 with 8x NVIDIA V100 GPUs 32GB).}
\label{fig:batch_imagenet}
\end{figure*}



==> Frivolous-AAAI-source(1)/tex_figures/supp_data_mlp.tex <==
\begin{figure*}[h!]
\centering
\begin{tabular}{cc}
	\includegraphics[width=.4\linewidth]{figures/acc_synth_data_test.pdf}&
	\includegraphics[width=.4\linewidth]{figures/auc_synthetic_data_test.pdf}\\
	(a) & (b)\\
	\includegraphics[width=.4\linewidth]{figures/comp_synthetic_data_test.pdf} &
	\includegraphics[width=.4\linewidth]{figures/sim_synth_data_test.pdf} \\
	(c) & (d)\\
\end{tabular}
\caption{\textbf{Varying training set size only affects compressibility amount in MLPs (Uncorrelated 10,000 dimensional synthetic data).} Trends in (a) accuracy, (b) robustness, (c) compressibility, and (d) similarity with various numbers of training examples across size factors for MLPs trained on 10,000 dimensional synthetic uncorrelated data.}
\label{fig:data_mlp}
\end{figure*}


==> Frivolous-AAAI-source(1)/tex_figures/supp_dynamics_imagenet.tex <==
\begin{figure*}[]
\centering
\begin{tabular}{ccc}
	\includegraphics[width=.3\linewidth]{figs/acc_imagenet_dynamics_test.pdf}&
	\includegraphics[width=.3\linewidth]{figs/prune_imagenet_dynamics.pdf} &
	% \includegraphics[width=.4\linewidth]{figures/comp_imagenet_dynamics_test.pdf} & 
	\includegraphics[width=.3\linewidth]{figs/red_imagenet_dynamics.pdf}\\
	(a) & (b) & (c)\\
\end{tabular}
\caption{Prunability and redundancy are stable in ResNet18s under different numbers of training epochs past convergence. Trends in (a) accuracy, (b) prunability, and (c) redundancy across training epochs after convergence.}
\label{fig:dynamics}
\end{figure*}

==> Frivolous-AAAI-source(1)/tex_figures/supp_init2_mlp.tex <==
\begin{figure*}[]
\centering
\begin{tabular}{ccc}
	\includegraphics[width=.3\linewidth]{figs/acc_synth_10k_initializer_test.pdf}&
	\includegraphics[width=.3\linewidth]{figs/prune_synth_10k_initializer.pdf} &
	% \includegraphics[width=.4\linewidth]{figures/comp_synthetic_inits_test.pdf} &
	\includegraphics[width=.3\linewidth]{figs/red_synth_10k_initializer.pdf} \\
	(a) & (b) & (c)\\
\end{tabular}
\caption{Redundancy is sensitive to initialization variance in MLPs trained on 10,000 dimensional data. Trends in (a) accuracy, (b) prunability, and (c) redundancy with multiple initialization variances across size factors for MLPs trained on synthetic uncorrelated data. The legend gives standard deviations for the Gaussian initialization. Redundancy is sensitive to initialization variance with the smallest variances resulting in the greatest amounts of redundancy.}
\label{fig:init_mlp}
\end{figure*}

==> Frivolous-AAAI-source(1)/tex_figures/supp_inits_cifar.tex <==
\begin{figure*}[]
\centering
\begin{tabular}{ccc}
	\includegraphics[width=.3\linewidth]{figs/acc_cifar_initializers2_test.pdf}&
	\includegraphics[width=.3\linewidth]{figs/prune_cifar_initializers_uni.pdf} &
	% \includegraphics[width=.4\linewidth]{figures/comp_cifar_initializers2_test.pdf} &
	\includegraphics[width=.3\linewidth]{figs/red_cifar_initializers_uni.pdf} \\
	(a) & (b) & (c)\\
\end{tabular}
\caption{AlexNet prunability and redundancy trends with uniform initializations (CIFAR-10). Trends in (a) accuracy, (b) prunability, and (c) redundancy with Glorot, He, and LeCun uniform initializations across size factors for AlexNets. Trends resemble those for Gaussian initializations.}
\label{fig:init_cifar}
\end{figure*}

==> Frivolous-AAAI-source(1)/tex_figures/supp_inits_mlp.tex <==
\begin{figure*}[]
\centering
\begin{tabular}{ccc}
	\includegraphics[width=.3\linewidth]{figs/acc_synth_10_initializer_test.pdf}&
	\includegraphics[width=.3\linewidth]{figs/prune_synth_10_initializer.pdf} &
	% \includegraphics[width=.4\linewidth]{figures/comp_synthetic_initializer2_test_10.pdf} &
	\includegraphics[width=.3\linewidth]{figs/red_synth_10_initializer.pdf} \\
	(a) & (b) & (c)\\
\end{tabular}
\caption{Frivolous units are not sensitive to initialization variance in MLPs trained on 10 dimensional data. Trends in (a) accuracy, (b) prunability, and (c) redundancy with multiple initialization variances across size factors for MLPs trained on synthetic uncorrelated data. The legend gives standard deviations for the Gaussian initialization.}
\label{fig:init_mlp_old}
\end{figure*}

==> Frivolous-AAAI-source(1)/tex_figures/supp_optim_mlp.tex <==
\begin{figure*}[]
\centering
\begin{tabular}{ccc}
	\includegraphics[width=.3\linewidth]{figs/acc_synth_10k_optimizer_test.pdf}&
	\includegraphics[width=.3\linewidth]{figs/prune_synth_10k_optimizer.pdf}&
	% \includegraphics[width=.4\linewidth]{figures/comp_synthetic_optim_test.pdf} &
	\includegraphics[width=.3\linewidth]{figs/red_synth_10k_optimizer.pdf} \\
	(a) & (b) & (c) \\
\end{tabular}
\caption{Optimizers influence redundancy in MLPs trained on 10,000 dimensional uncorrelated data. Trends in (a) accuracy, (b) prunability, and (c) redundancy with momentum, stochastic gradient descent, and Adam optimizers across size factors. Momentum, marked in purple, was used for all other experiments with these MLPs. Notably, momentumless stochastic gradient descent resulted in the most redundancy.}
\label{fig:optim_mlp}
\end{figure*}


==> Frivolous-AAAI-source(1)/tex_figures/supp_randomlabels.tex <==

\begin{figure*}[t!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}

    \includegraphics[width=.26\linewidth,valign=T]{figs/prune_cifar_rand.pdf} & 
	\includegraphics[width=.26\linewidth,valign=T]{figs/prune_cifar_regularizers.pdf}&
	\includegraphics[width=.26\linewidth,valign=T]{figs/prune_cifar_initializers.pdf} &
	\includegraphics[width=.26\linewidth,valign=T]{figs/prune_synth_summary.pdf}\\%[-1em]

    \includegraphics[width=.26\linewidth]{figs/red_cifar_rand.pdf} & 
	\includegraphics[width=.26\linewidth]{figs/red_cifar_regularizers.pdf}&
	\includegraphics[width=.26\linewidth]{figs/red_cifar_initializers.pdf} &
	\includegraphics[width=.26\linewidth]{figs/red_synth_summary.pdf}\\
	
	(a) & (b)& (c)& (d)\\
	
\end{tabular}
\caption{Prunability and/or redundancy outpace the growth of the overall network for different architectures, regularizers, initializers and datasets. (a) AlexNets and ResNet56s trained with and without random labels (CIFAR-10). (b) AlexNets trained with and without regularization (CIFAR-10). (c) AlexNets trained with various initializations (CIFAR-10). (d) MLPs with different trainsets and initializations (synthetic data). Max and min gain factors are given for each plot.}
\label{fig:results_other}
\vspace*{-0.4cm}
\end{figure*}





==> Frivolous-AAAI-source(1)/tex_figures/supp_regularizers.tex <==
\begin{figure*}[h!]
\centering
\begin{tabular}{ccc}
	\includegraphics[width=.3\linewidth]{figures/acc_cifar_regularizers_test.pdf}&
	\includegraphics[width=.3\linewidth]{figures/auc_cifar_regularizers_test.pdf}&
	% \includegraphics[width=.4\linewidth]{figures/comp_cifar_regularizers_test.pdf} &
	\includegraphics[width=.3\linewidth]{figures/sim_cifar_regularizers_test.pdf} \\
	(a) & (b) & (c)\\
\end{tabular}
\caption{\textbf{Explicit regularization affects amounts but not trends for unit removability and similarity in AlexNets (CIFAR-10).} Trends in (a) accuracy, (b) removability, and (c) similarity with various explicit regularizers across size factors for AlexNets. We test data augmentation, dropout, weight decay, and all three together against the unregularized control. Each regularizer positively affects generalization performance, though weight decay only has a slightly positive effect. None serve to change the general trends in units removability and similarity, but they shift the curves up or down. Dropout and weight decay have a large and small positive effect on removability and similarity respectively. We attribute this to dropout forcing networks to develop redundant units to cope with ablations and weight decay pushing the weights of the network toward a smaller subspace.}
\label{fig:regs}
\end{figure*}


==> Frivolous-AAAI-source(1)/tex_figures/table_networks.tex <==

\begin{table*}
\footnotesize
\centering
\begin{tabular}{|llllll|}
\hline
\cellcolor{Gray}\textbf{Dataset} & \cellcolor{Gray}\textbf{Network} &
\cellcolor{Gray}\textbf{Initialization} &
\cellcolor{Gray}\textbf{Optimizer} &
\cellcolor{Gray}\textbf{Regularizers} &
\cellcolor{Gray}\textbf{L.Rate-B.Size} \\\hline

Uncorr. 10 dim &  MLP & Normal$\star$ & Momentum & None & Best  \\\hline
\multirow{2}{*}{Uncorr. 10k dim} &  \multirow{2}{*}{MLP} & \multirow{2}{*}{Normal$\star$} & Momentum, SGD& \multirow{2}{*}{None} & \multirow{2}{*}{Best}  \\
& & & Adam $\star$ & & \\\hline
\multirow{1}{*}{CIFAR-10} & AlexNet & Glorot/LeCun/He$\star$ & Momentum & None, DA, DO, WD$\star$ & Best$\star$  \\
\multirow{1}{*}{(+ rand. labels$\star$)} & ResNet56 & Glorot & Momentum & BN, DA, WD & Best$\star$ \\\hline
\multirow{2}{*}{ImageNet} & ResNet18 & Glorot & Momentum & BN, DA, WD& Best$\star$   \\
& Inception-v3 & Normal & RMSProp & BN, DA, WD  & Best  \\\hline

\end{tabular}
\caption{Network training and performance details: ``BN'' refers to batch normalization, ``DA'' refers to data augmentation, ``DO'' refers to dropout, and ``WD'' refers to L2 weight decay. ``Best'' refers to learning rate/batch size combinations that achieved the highest accuracy. Stars ($\star$) indicate factors for which we tested multiple hyperparameters/variants.}
\label{tbl:nets}
\end{table*}
\normalsize




==> Frivolous-AAAI-source(1)/tex_figures/violin.tex <==
\begin{figure*}[h!]
\centering
\includegraphics[width=1\linewidth]{figures/violin.pdf}
\caption{\textbf{Absolute value correlation coefficients between neurons in AlexNet models:} The columns correspond to unregularized, regularized (data augmentation, dropout, and weight decay), and random-label-fitting AlexNets in CIFAR-10. The rows correspond to hidden layers of the networks. The first two of which are convolutional and the last two fully connected. Blue bars give means. Each plot shows the distribution for the 1/4x, 1x, and 4x model sizes.}
\label{fig:violin}
\end{figure*}

==> tex_figures/ablation.tex <==
\begin{figure}[t!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{0.1cm}}c}
%	\includegraphics[width=.33\linewidth]{figures/rob_imagenet.pdf} &
  \includegraphics[width=.5\linewidth]{figures/rob_cifar.pdf} &
   \includegraphics[width=.5\linewidth]{figures/rob_cifar_init.pdf} \\
	(a) & (b) \\ 
\end{tabular}
\caption{\textbf{Some  networks  develop  more  resistance  to unit removal as model size increases.}  Each point shows the proportion of labels that did not change when the percentage of units on the x-axis were randomly ablated. Networks were identically trained except for initialization and model size. No explicit regularization was used. (a) Glorot-initialized AlexNets in CIFAR-10. (b) He-initialized AlexNets in CIFAR-10.}
\label{fig:ablation}
\end{figure}


\begin{figure}[t!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{0.1cm}}c}
%	\includegraphics[width=.33\linewidth]{figures/rob_imagenet.pdf} &
      	\includegraphics[width=.5\linewidth]{figures/glorot_violins.pdf} &
	\includegraphics[width=.5\linewidth]{figures/he_violins.pdf} \\
	(a) & (b)  \\ 
\end{tabular}
\caption{\textbf{Some networks develop more highly correlated units as model size increases.} Each violin plot shows the distribution of pairwise correlation coefficients for the final convolutional layer of the network across the testing set. Networks were identically trained except for initialization and model size. No explicit regularization was used. (a) Glorot-initialized AlexNets in CIFAR-10. (b) He-initialized AlexNets in CIFAR-10.}
\label{fig:ablation2}
\end{figure}


==> tex_figures/accuracy_train.tex <==
\begin{figure*}[h!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
	\includegraphics[width=.33\linewidth]{figures/acc_synth_train.pdf}&
	\includegraphics[width=.33\linewidth]{figures/acc_cifar_initializers_train.pdf} &
	\includegraphics[width=.33\linewidth]{figures/acc_imagenet_train.pdf}\\
	(a) & (b) & (c) \\
\end{tabular}
\caption{\textbf{Train accuracies for our featured networks:} Each point represents a mean top-1 accuracy. Error bars are too small to appear at this scale.}
\label{fig:trainaccuracy}
\end{figure*}

==> tex_figures/auc.tex <==
\begin{figure*}[h!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
	\includegraphics[width=.33\linewidth]{figures/auc_synthetic_test.pdf}&
	\includegraphics[width=.33\linewidth]{figures/auc_cifar_initializers_test.pdf} &
	\includegraphics[width=.33\linewidth]{figures/auc_imagenet_test.pdf}\\
	(a) & (b) & (c) \\
\end{tabular}
\caption{\textbf{Areas under random ablation curves:} For each non-ImageNet network, we trained three replicates, and each point is an average across layers, samplings, and replicates (if applicable). Most error bars are too small to appear at this scale. We attribute the fact that the smallest MLPs did not have 50\% label change after 100 \% ablation to our use of bias terms in each layer.}
\label{fig:auc}
\end{figure*}

==> tex_figures/compression.tex <==
\begin{figure*}[h!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
	\includegraphics[width=.33\linewidth]{figures/comp_synthetic_test.pdf}&
	\includegraphics[width=.33\linewidth]{figures/comp_cifar_initializers_test.pdf} &
	\includegraphics[width=.33\linewidth]{figures/comp_imagenet_test.pdf}\\
	(a) & (b) & (c) \\
\end{tabular}
\caption{\textbf{Compressibility:} What proportion of principle components (relative to the number of neurons) are needed to explain 95\% of the variance in the neuronal activation vectors. For each non-ImageNet network, we trained three replicates, and each point is an average across layers, samplings, and replicates (if applicable). Most error bars are too small to appear at this scale.}
\label{fig:compression}
\end{figure*}

==> tex_figures/non_selectivity.tex <==
\begin{figure}[h!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
	\includegraphics[width=.33\linewidth]{figures/noselec_synthetic_test.pdf}&
	\includegraphics[width=.33\linewidth]{figures/noselec_cifar_initializers_test.pdf} &
	\includegraphics[width=.33\linewidth]{figures/nonselec_imagenet_test.pdf}\\
	(a) & (b) & (c) \\
\end{tabular}
\caption{\textbf{Nonselectivity:} Proportions of neurons with a selectivity factor of less than 0.05 where 0 is perfect promiscuity and 1 is perfect selectivity. For each non-ImageNet network, we trained three replicates, and each point is an average across layers, samplings, and replicates (if applicable). Most error bars are too small to appear at this scale.}
\label{fig:nonselectivity}
\end{figure}

==> tex_figures/results_cifar.tex <==
\begin{figure}[t!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
  \includegraphics[width=.26\linewidth]{figures/nonprune_imagenet.pdf} &
  \includegraphics[width=.26\linewidth]{figures/nonred_imagenet.pdf} &
    \includegraphics[width=.26\linewidth]{figures/nonprune_cifar_regularizers.pdf} &
    \includegraphics[width=.26\linewidth]{figures/nonred_cifar_regularizers.pdf}\\
	(a) & (b) & (c) & (d)  \\
\end{tabular}
\caption{\textbf{Initialization influences unit removability and repetition.} Glorot initialization leads to repetition without replication, He initialization leads to repetition without removability, and LeCun initialization leads to intermediate results in AlexNets (CIFAR-10) (a) Areas under ablation curves, (b) the average number of similar units per unit. Each point is an average across layers.}

\label{fig:results_cifar}
\end{figure}


==> tex_figures/results_synthetic.tex <==
\begin{figure}[h!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
	\includegraphics[width=.33\linewidth]{figures/auc_synthetic_test.pdf} & 
	\includegraphics[width=.33\linewidth]{figures/comp_synthetic_test.pdf} & 
	\includegraphics[width=.33\linewidth]{figures/selec_synth_test.pdf}\\
	(a) & (b) & (c) \\
\end{tabular}
\caption{\textbf{Uncorrelated data MLP robustness and redundancy:} (a) Areas under ablation curves. (b) What proportion of principle components (relative to the number of neurons) are needed to explain 95\% of the variance in the neuronal activation vectors. (c) The average number of similar neurons (neurons with a Pearson $abs(r)$ of at least 0.5) per neuron in each model. Each point is an average across layers, samplings, and 3 model replicates. Each point is an average across layers, samplings, and three model replicates. For (a) and (b), error bars are based on replicates and are mostly too small to appear. For (c), error bars represent the average standard deviation of selectivity \emph{within} samplings.}
\label{fig:results_imagenet}
\end{figure}

==> tex_figures/selectivity.tex <==
\begin{figure}[h!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
	\includegraphics[width=.33\linewidth]{figures/selec_synth_test.pdf}&
	\includegraphics[width=.33\linewidth]{figures/selec_cifar_initializers_test.pdf} &
	\includegraphics[width=.33\linewidth]{figures/selec_imagenet_test.pdf}\\
	(a) & (b) & (c) \\
\end{tabular}
\caption{\textbf{Selectivity:} The average selectivity factor where 0 is perfect promiscuity and 1 is perfect selectivity. For each non-ImageNet network, we trained three replicates, and each point is an average across layers, samplings, and replicates (if applicable). Error bars represent the average standard deviation of selectivity \emph{within} samplings.}
\label{fig:selectivity}
\end{figure}

==> tex_figures/similarity.tex <==
\begin{figure*}[h!]
\centering
\begin{tabular}{@{\hspace{-0.2cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
	\includegraphics[width=.33\linewidth]{figures/sim_synth_test.pdf}&
	\includegraphics[width=.33\linewidth]{figures/sim_cifar_initializers_test.pdf} &
	\includegraphics[width=.33\linewidth]{figures/sim_imagenet_test.pdf}\\
	(a) & (b) & (c) \\
\end{tabular}
\caption{\textbf{Similarity:} The average number of similar neurons (neurons with a Pearson $abs(r)$ of at least 0.5) per neuron in each model. For each non-ImageNet network, we trained three replicates, and each point is an average across layers, samplings, and replicates (if applicable). Error bars represent the average standard deviation of similarity \emph{within} samplings.}
\label{fig:similarity}
\end{figure*}

==> tex_figures/supp_data_mlp.tex <==
\begin{figure*}[h!]
\centering
\begin{tabular}{cc}
	\includegraphics[width=.4\linewidth]{figures/acc_synth_data_test.pdf}&
	\includegraphics[width=.4\linewidth]{figures/auc_synthetic_data_test.pdf}\\
	(a) & (b)\\
	\includegraphics[width=.4\linewidth]{figures/comp_synthetic_data_test.pdf} &
	\includegraphics[width=.4\linewidth]{figures/sim_synth_data_test.pdf} \\
	(c) & (d)\\
\end{tabular}
\caption{\textbf{Varying training set size only affects compressibility amount in MLPs (Uncorrelated 10,000 dimensional synthetic data).} Trends in (a) accuracy, (b) robustness, (c) compressibility, and (d) similarity with various numbers of training examples across size factors for MLPs trained on 10,000 dimensional synthetic uncorrelated data.}
\label{fig:data_mlp}
\end{figure*}


==> tex_figures/supp_regularizers.tex <==
\begin{figure*}[h!]
\centering
\begin{tabular}{ccc}
	\includegraphics[width=.3\linewidth]{figures/acc_cifar_regularizers_test.pdf}&
	\includegraphics[width=.3\linewidth]{figures/auc_cifar_regularizers_test.pdf}&
	% \includegraphics[width=.4\linewidth]{figures/comp_cifar_regularizers_test.pdf} &
	\includegraphics[width=.3\linewidth]{figures/sim_cifar_regularizers_test.pdf} \\
	(a) & (b) & (c)\\
\end{tabular}
\caption{\textbf{Explicit regularization affects amounts but not trends for unit removability and similarity in AlexNets (CIFAR-10).} Trends in (a) accuracy, (b) removability, and (c) similarity with various explicit regularizers across size factors for AlexNets. We test data augmentation, dropout, weight decay, and all three together against the unregularized control. Each regularizer positively affects generalization performance, though weight decay only has a slightly positive effect. None serve to change the general trends in units removability and similarity, but they shift the curves up or down. Dropout and weight decay have a large and small positive effect on removability and similarity respectively. We attribute this to dropout forcing networks to develop redundant units to cope with ablations and weight decay pushing the weights of the network toward a smaller subspace.}
\label{fig:regs}
\end{figure*}


==> tex_figures/violin.tex <==
\begin{figure*}[h!]
\centering
\includegraphics[width=1\linewidth]{figures/violin.pdf}
\caption{\textbf{Absolute value correlation coefficients between neurons in AlexNet models:} The columns correspond to unregularized, regularized (data augmentation, dropout, and weight decay), and random-label-fitting AlexNets in CIFAR-10. The rows correspond to hidden layers of the networks. The first two of which are convolutional and the last two fully connected. Blue bars give means. Each plot shows the distribution for the 1/4x, 1x, and 4x model sizes.}
\label{fig:violin}
\end{figure*}
